Operations on Metric Thickenings

Many simplicial complexes arising in practice have an associated metric space structure on the vertex set but not on the complex, e.g. the Vietoris-Rips complex in applied topology. We formalize a remedy by introducing a category of simplicial metric thickenings whose objects have a natural realization as metric spaces. The properties of this category allow us to prove that, for a large class of thickenings including Vietoris-Rips and Cech thickenings, the product of metric thickenings is homotopy equivalent to the metric thickenings of product spaces, and similarly for wedge sums.

==> eptcsdata.tex <==
\providecommand{\firstpage}{261}
\providecommand{\publicationstatus}{David I. Spivak and Jamie Vicary (Eds.):\\
Applied Category Theory 2020 (ACT2020)\\
EPTCS 333, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.333.18}{10.4204/EPTCS.333.18}}
\pdfoutput=1

